Optimizing NILC Extractions of the Thermal Sunyaev-Zeldovich Effect with Deep Learning

All-sky maps of the thermal Sunyaev-Zel'dovich effect (SZ) tend to suffer from systematic features arising from the component separation techniques used to extract the signal. In this work, we investigate one of these methods known as needlet internal linear combination (NILC) and test its performance on simulated data. We show that NILC estimates are strongly affected by the choice of the spatial localization parameter ($\Gamma$), which controls a bias-variance trade-off. Typically, NILC extractions assume a fixed value of $\Gamma$ over the entire sky, but we show there exists an optimal $\Gamma$ that depends on the SZ signal strength and local contamination properties. Then we calculate the NILC solutions for multiple values of $\Gamma$ and feed the results into a neural network to predict the SZ signal. This extraction method, which we call Deep-NILC, is tested against a set of validation data, including recovered radial profiles of resolved systems. Our main result is that Deep-NILC offers significant improvements over choosing fixed values of $\Gamma$.

==> Abstract.tex <==
\begin{abstract}

Much of the baryons in galaxy groups are thought to have been driven out to large distances ($\gtrsim$\Rvir) by feedback, but there are few constraining observations of this extended gas. This work presents the resolved Sunyaev\textendash Zel'dovich (SZ) profiles for a stacked sample of 10 nearby galaxy groups within the mass range log$_{10}(M_{500}[M_{\odot}]) = 13.6 -13.9$. We measured the SZ profiles using the publicly available \ymap from the Planck Collaboration as well as our own \ymaps constructed from more recent versions of \Planck data. The \ymap extracted from the latest data release yielded a significant SZ detection out to 3 \Rvir. In addition, the stacked profile from these data \textbf{was} consistent with simulations that included AGN feedback. Our best-fit model using the latest \Planck data suggested a baryon fraction $\approx 5.6\%$ within \Rvir. This is significantly lower than the cosmic value of $\approx 16\%$, supporting the idea that baryons have been driven to large radii by AGN feedback. Lastly, we discovered a significant ($\sim 3\sigma$) ``bump'' feature near $\sim 2$ \Rvir that is most likely the signature of internal accretion shocks.

\end{abstract}


\keywords{Galaxy groups --- Sunyaev\textendash Zel'dovich effect --- Intracluster medium --- Active galactic nuclei}
